Blockchain based Resource Governance for Decentralized Web Environments

Decentralization initiatives such as Solid and ActivityPub aim to give data owners more control over their data and to level the playing field by enabling small companies and individuals to gain access to data, thus stimulating innovation. However, these initiatives typically employ access control mechanisms that cannot verify compliance with usage conditions after access has been granted to others. In this paper, we extend the state of the art by proposing a resource governance conceptual framework, entitled ReGov, that facilitates usage control in decentralized web environments. We subsequently demonstrate how our framework can be instantiated by combining blockchain and trusted execution environments. Through blockchain technologies, we record policies expressing the usage conditions associated with resources and monitor their compliance. Our instantiation employs trusted execution environments to enforce said policies, inside data consumers' devices.} We evaluate the framework instantiation through a detailed analysis of requirements derived from a data market motivating scenario, as well as an assessment of the security, privacy, and affordability aspects of our proposal.

==> content/DTindexing_table.tex <==
%
% !TeX root = ../main.tex
% !TeX spellcheck = en_US
%
\begin{table}[]
\centering
\scriptsize
\resizebox{\columnwidth}{!}{%
\tabulinesep=0.7 mm
\begin{tabu}{|l|}
\hline
\multicolumn{1}{|c|}{DTindexing extends Ownable}                                                \\ \hline
private podsCounter: int                                                                                                                        \\
private resourceCounter: int                                                                                                                    \\
private dtSubscription: int                                                                                                                     \\
private podList: Pod{[}{]}                                                                                                                      \\
private resourceList: Resource{[}{]}                                                                                                            \\ \hline
private searchByType(tp: PodType): Pod{[}{]}                                                                                                    \\
{\guillemotleft}event{\guillemotright} NewPod(idPod: int, obgliationAddress: address)                                            \\
\textless{}\textless{}event\textgreater{}\textgreater NewResource(idResource: int)                                                              \\
\textless{}\textless{}modifier\textgreater{}\textgreater validPodId(id: uint, owner: address)                                                   \\
public getMedicalPods(idSubscription: uint): Pod{[}{]}                                                                                          \\
public getSocialPods(idSubscription: uint): Pod{[}{]}                                                                                           \\
public getFinancialPods(idSubscription: uint): Pod{[}{]}                                                                                        \\
public registerPod(newReferene: bytes, podType: PodType, podAddress: address): int                                                              \\
public registerResource(podId: int, newReferene: bytes, idSubscription: uint): int \textless{}\textless{}validPodId\textgreater{}\textgreater{} \\
public getPodResources(podId: int, idSubscription: int): Resource{[}{]}                                                                         \\
public getResource(idResource: int): Resource \textless{}\textless{}validResourceId\textgreater{}\textgreater{}                                 \\
public deactivateResource(idResource: int): Resource \textless{}\textless{}validResourceId\textgreater{}\textgreater{}                          \\ \hline
\end{tabu}
}
\caption{Class diagram of the DTindexing smart contract.}
\end{table}

==> content/DTobligations_table.tex <==
%
% !TeX root = ../main.tex
% !TeX spellcheck = en_US
%
\begin{table}[]
\centering
\footnotesize
\resizebox{\columnwidth}{!}{%
\tabulinesep=0.7 mm
\begin{tabu}{|l|}
\hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}DTobligations \\ \textless{}\textless{}extends\textgreater{}\textgreater Ownable\end{tabular}}                                    \\ \hline
dtIndexing: DTindexing                                                                                                                                                            \\
defaultPodObligation: ObligationRules                                                                                                                                             \\
resourcesObligation: mapping(int=\textgreater{}ObligationRules)                                                                                                                   \\ \hline
\textless{}\textless{}modifier\textgreater{}\textgreater hasSpecificRules(resourceId: int)                                                                                        \\
\textless{}\textless{}modifier\textgreater{}\textgreater isValidTemporal(deadline: uint)                                                                                          \\
\textless{}\textless{}modifier\textgreater{}\textgreater isTheResourceCovered(idResource: int)                                                                                    \\
public constructor(dtInd: address, podAddress: address)                                                                                                                           \\
public getObligationRules(idResource: int): ObligationRules \textless{}\textless{}isTheResourceCovered\textgreater{}\textgreater{}                                                \\
public getDefaultObligationRules(): ObligationRules                                                                                                                               \\
public addDefaultAccessCounterObligation(accessCounter: uint)                                                                                                                     \\
public addDefaultTemporalObligation(temporalObligation: uint) \textless{}\textless{}isValidTemporal, onlyOwner\textgreater{}\textgreater{}                                        \\
public addDefaultCountryObligation(country: uint) \textless{}\textless{}onlyOwner\textgreater{}\textgreater{}                                                                     \\
public addDefaultDomainObligation(domain: DomainType) \textless{}\textless{}onlyOwner\textgreater{}\textgreater{}                                                                 \\
public addAccessCounterObligation(idResource: int, accessCounter: uint): ObligationRules \textless{}\textless{}isTheResourceCovered, onlyOwner\textgreater{}\textgreater{}        \\
public addDomainObligation(idResource: int, domain: DomainType): ObligationRules \textless{}\textless{}onlyOwner, isTheResourceCovered\textgreater{}\textgreater{}                \\
public addCountryObligation(idResource: int, country: uint): ObligationRules \textless{}\textless{}onlyOwner, isTheResourceCovered\textgreater{}\textgreater{}                    \\
public addTemporalObligation(idResource: int, deadline: uint): ObligationRules \textless{}\textless{}onlyOwner, isTheResourceCovered, isValidTemporal\textgreater{}\textgreater{} \\
public removeAccessCounterObligation(idResource: int) \textless{}\textless{}onlyOwner, isTheResourceCovered, hasSpecificRules\textgreater{}\textgreater{}                         \\
public removeTemporalObligation(idResource: int) \textless{}\textless{}isTheResourceCovered, onlyOwner, hasSpecificRules\textgreater{}\textgreater{}                              \\
public removeDomainObligation(idResource: int) \textless{}\textless{}isTheResourceCovered, onlyOwner, hasSpecificRules\textgreater{}\textgreater{}                                \\
public removeCountryObligation(idResource: int) \textless{}\textless{}isTheResourceCovered, onlyOwner, hasSpecificRules\textgreater{}\textgreater{}                               \\
public removeDefaultTemporalObligation() \textless{}\textless{}onlyOwner\textgreater{}\textgreater{}                                                                              \\
public removeDefaultAccessCounterObligation() \textless{}\textless{}onlyOwner\textgreater{}\textgreater{}                                                                         \\
public removeDefaultCountryObligation() \textless{}\textless{}onlyOwner\textgreater{}\textgreater{}                                                                               \\
public removeDefaultDomainObligation() \textless{}\textless{}onlyOwner\textgreater{}\textgreater{}                                                                                \\
public withSpecificRules(idResource: int): bool                                                                                                                                   \\
public monitorCompliance() \textless{}\textless{}onlyOwner\textgreater{}\textgreater{}                                                                                            \\ \hline
\end{tabu}
}
\caption{Class diagram of the DTindexing smart contract.}
\end{table}

==> content/related_works.tex <==
%
% !TeX root = ../main.tex
% !TeX spellcheck = en_US
%
\subsection{Related work}
\label{sec:rw}

Several works strive to provide more control and transparency with respect to personal data processing by leveraging blockchain distributed application platforms~\citep{DBLP:books/sp/XuWS19}. For instance, ~\citet{IoTBlock} defines an access control mechanism for IoT devices that stores a hash of the data in a blockchain infrastructure and maintains the raw information in a secure storage platform using a TEE.
In the proposed framework, a blockchain based ledger is used in order to develop an audit trail of data access that provides more transparency with respect to data processing. 
\cite{10.1007/978-3-030-59013-0_30} propose a system, called PrivacyGuard, which gives data owners control over personal data access and usage in a data market scenario.

The literature offers numerous study cases in which usage control frameworks have been instantiated to increase the degree of privacy and confidentiality of shared data.
\citet{neisseUsage} propose a usage control framework in which a Policy Enforcement Point (PEP) keeps track of business operations and intercepts action requests while taking into consideration Policy Decision Point event subscriptions (PDP). \citet{bai2014context} addresses usage control in a Web Of Thing environment by adapting the UCON model for Smart Home ecosystems. \citet{8936349} introduce a secure usage control scheme for Internet of things (IoT) data that is built upon a blockchain-based trust management approach. While, ~\citet{DBLP:journals/winet/KhanZSAM20} conceptualizes a distributed usage control model, named DistU, for industrial blockchain frameworks with monitoring procedures that are able to automatically revoke permissions.


Additionally, there are several papers that propose frameworks or architectures that combine  blockchain platforms and decentralized web initiatives such as Solid web. ~\citet{10.1145/3366424.3385759} demonstrate how together Solid data stores (i.e., pods) and blockchains can be used for trustless verification with confidentiality. \citet{patel2019dauth} propose a fully decentralized protocol named DAuth that leverage asymmetric encryption in order to implement authentication. While, \citet{9064776} introduce a secure Solid authentication mechanism, integrating Rivest–Shamir–Adleman (RSA) signatures into permissioned blockchain systems. In turn, ~\citet{DBLP:conf/esws/BeckerVKBK21} demonstrate how data stored in Solid pods can be monetized by leveraging a blockchain based payment system. Whereas, ~\citet{havur2020greater} discuss how solid could potentially leverage existing consent, transparency and compliance checking approaches. 

Many studies have shown that blockchain and TEEs can profitably coexist. The state of the art proposes numerous cases where the combination of the two technologies leads to advantages in terms of data ownership, availability, and trust. One of these is the work of \citet{liang2017towards}, that propose a patient-centric personal health data management system with accountability and decentralization. The architecture of the framework employs TEEs to generate a fingerprint for each data access that are immutably maintained by a blockchain infrastructure. Whereas, \citet{lind2017teechain} designed and implemented a protocol named Teechain that integrates off-chain TEEs for secure and scalable payment procedures, built on top of the Bitcoin blockchain platform.

As the decentralized web continues to gain momentum in providing users with greater autonomy over their personal resources, there is a need to address the limitations in current access control methods. These simple mechanisms, while effective in managing access, are not sufficient in ensuring that usage conditions are upheld post-access.

